The Rise and Fall of Debris Disks: MIPS Observations of h and chi Persei and the Evolution of Mid-IR Emission from Planet Formation

We describe Spitzer/MIPS observations of the double cluster, h and $\chi$ Persei, covering a $\sim$ 0.6 square-degree area surrounding the cores of both clusters. The data are combined with IRAC and 2MASS data to investigate $\sim$ 616 sources from 1.25-24 $\mu m$. We use the long-baseline $K_{s}$-[24] color to identify two populations with IR excess indicative of circumstellar material: Be stars with 24 $\mu m$ excess from optically-thin free free emission and 17 fainter sources (J$\sim$ 14-15) with [24] excess consistent with a circumstellar disk. The frequency of IR excess for the fainter sources increases from 4.5 $\mu m$ through 24 $\mu m$. The IR excess is likely due to debris from the planet formation process. The wavelength-dependent behavior is consistent with an inside-out clearing of circumstellar disks. A comparison of the 24 $\mu m$ excess population in h and $\chi$ Per sources with results for other clusters shows that 24 $\mu m$ emission from debris disks 'rises' from 5 to 10 Myr, peaks at $\sim$ 10-15 Myr, and then 'falls' from $\sim$ 15/20 Myr to 1 Gyr.

==> tab1f.tex <==
\begin{deluxetable}{lllllllllllllll}
\tiny
%\rotate
%\documentstyle[10pt]
%SPMquot"(0pt)
%\setlength{\tabcolstep}{0.02in}
%\linewidth{0.1 in}
\tabletypesize{\tiny}
%\tabletypesize{\scriptsize}
\tablecolumns{18}
\tablecaption{MIPS sources with optical and 2MASS/IRAC counterparts in h \& $\chi$ Persei}
\tiny
\tablehead{{$\alpha$}&{$\delta$}&{V}&{B-V}&{U-B}&{J}&{H}&{$K_{s}$}&{[3.6]}&{[4.5]}&{[5.8]}&{[8]}&{\textbf{[24]}}&{$\sigma$([3.6])}&{$\sigma$([4.5])}&{$\sigma$([5.8])}&{$\sigma$([8])}&{\textbf{$\sigma$([24])}}}
\startdata

\enddata
\tablecomments{First five entries in our photometry catalogue from MIPS, 2MASS and IRAC.  Errors in the 
2MASS JH$K_{s}$ filters are $\lesssim$ 0.05 for sources except the $\sim$ 21 fainter (J$\sim$ 14-15) sources.
Values of 99.0 or -100.00 denote sources that were not observed in the given filter at the 5$\sigma$ level.}
\end{deluxetable}

